Learning-Based Rich Feedback HARQ for Energy-Efficient Uplink Short Packet Transmission

The trade-off between reliability, latency, and energy efficiency is a central problem in communication systems. Advanced hybrid automated repeat request (HARQ) techniques reduce retransmissions required for reliable communication but incur high computational costs. Strict energy constraints apply mainly to devices, while the access point receiving their packets is usually connected to the electrical grid. Therefore, moving the computational complexity from the transmitter to the receiver may provide a way to improve this trade-off. We propose the reinforcement-based adaptive feedback (RAF) scheme, a departure from traditional single-bit feedback HARQ, introducing adaptive rich feedback where the receiver requests the coded retransmission of specific symbols. Simulation results show that RAF achieves a better trade-off between energy efficiency, reliability, and latency, compared to existing HARQ solutions. Our RAF scheme can easily adapt to different modulation schemes and can also generalize to different channel statistics.

==> tikzplotlib_figs_icmlcn/256QAM_Pareto_Lp1_data.tex <==
\path [draw=color1, very thin]
(axis cs:1.05346666666667,0)
--(axis cs:1.05346666666667,31.661378838055)
--(axis cs:1.0602,31.661378838055)
--(axis cs:1.0602,31.9014035856142)
--(axis cs:1.08173333333333,31.9014035856142)
--(axis cs:1.08173333333333,32.0784218610387)
--(axis cs:1.0969,32.0784218610387)
--(axis cs:1.0969,32.3467175210818)
--(axis cs:1.1189,32.3467175210818)
--(axis cs:1.1189,32.6633390372418)
--(axis cs:1.14463333333333,32.6633390372418)
--(axis cs:1.14463333333333,33.0526167199646)
--(axis cs:1.1878,33.0526167199646)
--(axis cs:1.1878,33.441795966977)
--(axis cs:1.25976666666667,33.441795966977)
--(axis cs:1.25976666666667,33.8143858112075)
--(axis cs:1.3547,33.8143858112075)
--(axis cs:1.3547,34.3669272020491)
--(axis cs:1.50436666666667,34.3669272020491)
--(axis cs:1.50436666666667,34.8543582781167)
--(axis cs:1.72773333333333,34.8543582781167)
--(axis cs:1.72773333333333,35.3986574961204)
--(axis cs:2.071,35.3986574961204)
--(axis cs:2.071,35.8812481440104)
--(axis cs:2.6225,35.8812481440104)
--(axis cs:2.6225,36.0904369107464)
--(axis cs:2.6225,36.0904369107464)
--(axis cs:2.6225,36.0904369107464)
--(axis cs:4.6225,36.0904369107464)
--(axis cs:4.6225,36.0904369107464)
--(axis cs:4.6225,36.0904369107464)
--(axis cs:4.6225,0);

\path [draw=color1, fill=color1, opacity=0.1, very thin]
(axis cs:1.05346666666667,0)
--(axis cs:1.05346666666667,31.661378838055)
--(axis cs:1.0602,31.661378838055)
--(axis cs:1.0602,31.9014035856142)
--(axis cs:1.08173333333333,31.9014035856142)
--(axis cs:1.08173333333333,32.0784218610387)
--(axis cs:1.0969,32.0784218610387)
--(axis cs:1.0969,32.3467175210818)
--(axis cs:1.1189,32.3467175210818)
--(axis cs:1.1189,32.6633390372418)
--(axis cs:1.14463333333333,32.6633390372418)
--(axis cs:1.14463333333333,33.0526167199646)
--(axis cs:1.1878,33.0526167199646)
--(axis cs:1.1878,33.441795966977)
--(axis cs:1.25976666666667,33.441795966977)
--(axis cs:1.25976666666667,33.8143858112075)
--(axis cs:1.3547,33.8143858112075)
--(axis cs:1.3547,34.3669272020491)
--(axis cs:1.50436666666667,34.3669272020491)
--(axis cs:1.50436666666667,34.8543582781167)
--(axis cs:1.72773333333333,34.8543582781167)
--(axis cs:1.72773333333333,35.3986574961204)
--(axis cs:2.071,35.3986574961204)
--(axis cs:2.071,35.8812481440104)
--(axis cs:2.6225,35.8812481440104)
--(axis cs:2.6225,36.0904369107464)
--(axis cs:2.6225,36.0904369107464)
--(axis cs:2.6225,36.0904369107464)
--(axis cs:4.6225,36.0904369107464)
--(axis cs:4.6225,36.0904369107464)
--(axis cs:4.6225,0)
--(axis cs:4.6225,0)
--(axis cs:4.6225,0)
--(axis cs:2.6225,0)
--(axis cs:2.6225,0)
--(axis cs:2.6225,0)
--(axis cs:2.6225,0)
--(axis cs:2.071,0)
--(axis cs:2.071,0)
--(axis cs:1.72773333333333,0)
--(axis cs:1.72773333333333,0)
--(axis cs:1.50436666666667,0)
--(axis cs:1.50436666666667,0)
--(axis cs:1.3547,0)
--(axis cs:1.3547,0)
--(axis cs:1.25976666666667,0)
--(axis cs:1.25976666666667,0)
--(axis cs:1.1878,0)
--(axis cs:1.1878,0)
--(axis cs:1.14463333333333,0)
--(axis cs:1.14463333333333,0)
--(axis cs:1.1189,0)
--(axis cs:1.1189,0)
--(axis cs:1.0969,0)
--(axis cs:1.0969,0)
--(axis cs:1.08173333333333,0)
--(axis cs:1.08173333333333,0)
--(axis cs:1.0602,0)
--(axis cs:1.0602,0)
--(axis cs:1.05346666666667,0)
--cycle;

\path [draw=color2, very thin]
(axis cs:1.02033333333333,0)
--(axis cs:1.02033333333333,31.1088042357404)
--(axis cs:1.0459,31.1088042357404)
--(axis cs:1.0459,31.9405535462381)
--(axis cs:1.08046666666667,31.9405535462381)
--(axis cs:1.08046666666667,32.7814267565152)
--(axis cs:1.1284,32.7814267565152)
--(axis cs:1.1284,33.6175489489335)
--(axis cs:1.19126666666667,33.6175489489335)
--(axis cs:1.19126666666667,34.4512486554352)
--(axis cs:1.41623333333333,34.4512486554352)
--(axis cs:1.41623333333333,35.2700519605274)
--(axis cs:1.59433333333333,35.2700519605274)
--(axis cs:1.59433333333333,35.9033177218982)
--(axis cs:1.82656666666667,35.9033177218982)
--(axis cs:1.82656666666667,36.3583331049908)
--(axis cs:2.09896666666667,36.3583331049908)
--(axis cs:2.09896666666667,36.6566087898538)
--(axis cs:2.09896666666667,36.6566087898538)
--(axis cs:2.09896666666667,36.6566087898538)
--(axis cs:4.09896666666667,36.6566087898538)
--(axis cs:4.09896666666667,36.6566087898538)
--(axis cs:4.09896666666667,36.6566087898538)
--(axis cs:4.09896666666667,0);

\path [draw=color2, fill=color2, opacity=0.1, very thin]
(axis cs:1.02033333333333,0)
--(axis cs:1.02033333333333,31.1088042357404)
--(axis cs:1.0459,31.1088042357404)
--(axis cs:1.0459,31.9405535462381)
--(axis cs:1.08046666666667,31.9405535462381)
--(axis cs:1.08046666666667,32.7814267565152)
--(axis cs:1.1284,32.7814267565152)
--(axis cs:1.1284,33.6175489489335)
--(axis cs:1.19126666666667,33.6175489489335)
--(axis cs:1.19126666666667,34.4512486554352)
--(axis cs:1.41623333333333,34.4512486554352)
--(axis cs:1.41623333333333,35.2700519605274)
--(axis cs:1.59433333333333,35.2700519605274)
--(axis cs:1.59433333333333,35.9033177218982)
--(axis cs:1.82656666666667,35.9033177218982)
--(axis cs:1.82656666666667,36.3583331049908)
--(axis cs:2.09896666666667,36.3583331049908)
--(axis cs:2.09896666666667,36.6566087898538)
--(axis cs:2.09896666666667,36.6566087898538)
--(axis cs:2.09896666666667,36.6566087898538)
--(axis cs:4.09896666666667,36.6566087898538)
--(axis cs:4.09896666666667,36.6566087898538)
--(axis cs:4.09896666666667,0)
--(axis cs:4.09896666666667,0)
--(axis cs:4.09896666666667,0)
--(axis cs:2.09896666666667,0)
--(axis cs:2.09896666666667,0)
--(axis cs:2.09896666666667,0)
--(axis cs:2.09896666666667,0)
--(axis cs:1.82656666666667,0)
--(axis cs:1.82656666666667,0)
--(axis cs:1.59433333333333,0)
--(axis cs:1.59433333333333,0)
--(axis cs:1.41623333333333,0)
--(axis cs:1.41623333333333,0)
--(axis cs:1.19126666666667,0)
--(axis cs:1.19126666666667,0)
--(axis cs:1.1284,0)
--(axis cs:1.1284,0)
--(axis cs:1.08046666666667,0)
--(axis cs:1.08046666666667,0)
--(axis cs:1.0459,0)
--(axis cs:1.0459,0)
--(axis cs:1.02033333333333,0)
--cycle;

\path [draw=color3, very thin]
(axis cs:1.02323333333333,0)
--(axis cs:1.02323333333333,31.2841153761264)
--(axis cs:1.04853333333333,31.2841153761264)
--(axis cs:1.04853333333333,32.1308208687421)
--(axis cs:1.07906666666667,32.1308208687421)
--(axis cs:1.07906666666667,33.0141913806432)
--(axis cs:1.1356,33.0141913806432)
--(axis cs:1.1356,33.8220573770613)
--(axis cs:1.20583333333333,33.8220573770613)
--(axis cs:1.20583333333333,34.6266925545172)
--(axis cs:1.43636666666667,34.6266925545172)
--(axis cs:1.43636666666667,35.5070956874785)
--(axis cs:1.6342,35.5070956874785)
--(axis cs:1.6342,36.1226329985936)
--(axis cs:1.88833333333333,36.1226329985936)
--(axis cs:1.88833333333333,36.5328979733136)
--(axis cs:2.19366666666667,36.5328979733136)
--(axis cs:2.19366666666667,36.7691419299474)
--(axis cs:2.54313333333333,36.7691419299474)
--(axis cs:2.54313333333333,36.807712239561)
--(axis cs:2.54313333333333,36.807712239561)
--(axis cs:2.54313333333333,36.807712239561)
--(axis cs:4.54313333333333,36.807712239561)
--(axis cs:4.54313333333333,36.807712239561)
--(axis cs:4.54313333333333,36.807712239561)
--(axis cs:4.54313333333333,0);

\path [draw=color3, fill=color3, opacity=0.1, very thin]
(axis cs:1.02323333333333,0)
--(axis cs:1.02323333333333,31.2841153761264)
--(axis cs:1.04853333333333,31.2841153761264)
--(axis cs:1.04853333333333,32.1308208687421)
--(axis cs:1.07906666666667,32.1308208687421)
--(axis cs:1.07906666666667,33.0141913806432)
--(axis cs:1.1356,33.0141913806432)
--(axis cs:1.1356,33.8220573770613)
--(axis cs:1.20583333333333,33.8220573770613)
--(axis cs:1.20583333333333,34.6266925545172)
--(axis cs:1.43636666666667,34.6266925545172)
--(axis cs:1.43636666666667,35.5070956874785)
--(axis cs:1.6342,35.5070956874785)
--(axis cs:1.6342,36.1226329985936)
--(axis cs:1.88833333333333,36.1226329985936)
--(axis cs:1.88833333333333,36.5328979733136)
--(axis cs:2.19366666666667,36.5328979733136)
--(axis cs:2.19366666666667,36.7691419299474)
--(axis cs:2.54313333333333,36.7691419299474)
--(axis cs:2.54313333333333,36.807712239561)
--(axis cs:2.54313333333333,36.807712239561)
--(axis cs:2.54313333333333,36.807712239561)
--(axis cs:4.54313333333333,36.807712239561)
--(axis cs:4.54313333333333,36.807712239561)
--(axis cs:4.54313333333333,0)
--(axis cs:4.54313333333333,0)
--(axis cs:4.54313333333333,0)
--(axis cs:2.54313333333333,0)
--(axis cs:2.54313333333333,0)
--(axis cs:2.54313333333333,0)
--(axis cs:2.54313333333333,0)
--(axis cs:2.19366666666667,0)
--(axis cs:2.19366666666667,0)
--(axis cs:1.88833333333333,0)
--(axis cs:1.88833333333333,0)
--(axis cs:1.6342,0)
--(axis cs:1.6342,0)
--(axis cs:1.43636666666667,0)
--(axis cs:1.43636666666667,0)
--(axis cs:1.20583333333333,0)
--(axis cs:1.20583333333333,0)
--(axis cs:1.1356,0)
--(axis cs:1.1356,0)
--(axis cs:1.07906666666667,0)
--(axis cs:1.07906666666667,0)
--(axis cs:1.04853333333333,0)
--(axis cs:1.04853333333333,0)
--(axis cs:1.02323333333333,0)
--cycle;

\path [draw=color4, very thin]
(axis cs:1.0659,0)
--(axis cs:1.0659,31.5688015430916)
--(axis cs:1.0659,31.8744987758211)
--(axis cs:1.07476666666667,31.8744987758211)
--(axis cs:1.07476666666667,32.0902254736032)
--(axis cs:1.0987,32.0902254736032)
--(axis cs:1.0987,32.2880831643437)
--(axis cs:1.11123333333333,32.2880831643437)
--(axis cs:1.11123333333333,32.5442801875427)
--(axis cs:1.1398,32.5442801875427)
--(axis cs:1.1398,32.8683559246127)
--(axis cs:1.1717,32.8683559246127)
--(axis cs:1.1717,33.1894196718156)
--(axis cs:1.21303333333333,33.1894196718156)
--(axis cs:1.21303333333333,33.631997437391)
--(axis cs:1.2824,33.631997437391)
--(axis cs:1.2824,34.0394339043486)
--(axis cs:1.37866666666667,34.0394339043486)
--(axis cs:1.37866666666667,34.5639534557646)
--(axis cs:1.5494,34.5639534557646)
--(axis cs:1.5494,35.1123060520478)
--(axis cs:1.79846666666667,35.1123060520478)
--(axis cs:1.79846666666667,35.649275102528)
--(axis cs:2.17126666666667,35.649275102528)
--(axis cs:2.17126666666667,36.0633517325442)
--(axis cs:2.74356666666667,36.0633517325442)
--(axis cs:2.74356666666667,36.2558436194443)
--(axis cs:2.74356666666667,36.2558436194443)
--(axis cs:2.74356666666667,36.2558436194443)
--(axis cs:12.7435666666667,36.2558436194443)
--(axis cs:12.7435666666667,36.2558436194443)
--(axis cs:12.7435666666667,36.2558436194443)
--(axis cs:12.7435666666667,0);
\path [draw=color4, fill=color4, opacity=0.1, very thin]
(axis cs:1.0659,0)
--(axis cs:1.0659,31.5688015430916)
--(axis cs:1.0659,31.8744987758211)
--(axis cs:1.07476666666667,31.8744987758211)
--(axis cs:1.07476666666667,32.0902254736032)
--(axis cs:1.0987,32.0902254736032)
--(axis cs:1.0987,32.2880831643437)
--(axis cs:1.11123333333333,32.2880831643437)
--(axis cs:1.11123333333333,32.5442801875427)
--(axis cs:1.1398,32.5442801875427)
--(axis cs:1.1398,32.8683559246127)
--(axis cs:1.1717,32.8683559246127)
--(axis cs:1.1717,33.1894196718156)
--(axis cs:1.21303333333333,33.1894196718156)
--(axis cs:1.21303333333333,33.631997437391)
--(axis cs:1.2824,33.631997437391)
--(axis cs:1.2824,34.0394339043486)
--(axis cs:1.37866666666667,34.0394339043486)
--(axis cs:1.37866666666667,34.5639534557646)
--(axis cs:1.5494,34.5639534557646)
--(axis cs:1.5494,35.1123060520478)
--(axis cs:1.79846666666667,35.1123060520478)
--(axis cs:1.79846666666667,35.649275102528)
--(axis cs:2.17126666666667,35.649275102528)
--(axis cs:2.17126666666667,36.0633517325442)
--(axis cs:2.74356666666667,36.0633517325442)
--(axis cs:2.74356666666667,36.2558436194443)
--(axis cs:2.74356666666667,36.2558436194443)
--(axis cs:2.74356666666667,36.2558436194443)
--(axis cs:12.7435666666667,36.2558436194443)
--(axis cs:12.7435666666667,36.2558436194443)
--(axis cs:12.7435666666667,0)
--(axis cs:12.7435666666667,0)
--(axis cs:12.7435666666667,0)
--(axis cs:2.74356666666667,0)
--(axis cs:2.74356666666667,0)
--(axis cs:2.74356666666667,0)
--(axis cs:2.74356666666667,0)
--(axis cs:2.17126666666667,0)
--(axis cs:2.17126666666667,0)
--(axis cs:1.79846666666667,0)
--(axis cs:1.79846666666667,0)
--(axis cs:1.5494,0)
--(axis cs:1.5494,0)
--(axis cs:1.37866666666667,0)
--(axis cs:1.37866666666667,0)
--(axis cs:1.2824,0)
--(axis cs:1.2824,0)
--(axis cs:1.21303333333333,0)
--(axis cs:1.21303333333333,0)
--(axis cs:1.1717,0)
--(axis cs:1.1717,0)
--(axis cs:1.1398,0)
--(axis cs:1.1398,0)
--(axis cs:1.11123333333333,0)
--(axis cs:1.11123333333333,0)
--(axis cs:1.0987,0)
--(axis cs:1.0987,0)
--(axis cs:1.07476666666667,0)
--(axis cs:1.07476666666667,0)
--(axis cs:1.0659,0)
--(axis cs:1.0659,0)
--(axis cs:8.03683333333333,0)
--cycle;

\addplot [thick, color4]
table {%
-10 0
-9 0
};\label{plot:DHARQ}
\addplot [thick, color3]
table {%
-10 0
-9 0
};\label{plot:ST}
\addplot [thick, color2]
table {%
-10 0
-9 0
};\label{plot:HARQ}
\addplot [thick, color1]
table {%
-10 0
-9 0
};\label{plot:TA}


\addplot [semithick, color6, mark=diamond*, mark size=3, mark options={solid}, only marks]
table {%
1.6702 36.4261534016095
1.565967 36.2610163780905
1.6431 36.3924622908603
1.8841 36.5631334708683
1.811467 36.5203985377564
1.807267 36.5407277370851
1.929667 36.5374322994893
1.976 36.5926116460017
2.254867 36.5385669000209
};\label{plot:RAFalpha01}

\addplot [semithick, color5, mark=diamond*, mark size=3, mark options={solid}, only marks]
table {%
1.207367 34.8546098632158
1.246033 35.0844951665254
1.237533 35.034338080401
1.339867 35.5621729456748
1.29 35.2781967070258
1.381433 35.8248280712628
1.445867 35.6715662135164
1.552833 36.0728133507477
1.771867 36.3112985619421
};\label{plot:RAFalpha05}


==> tikzplotlib_figs_icmlcn/256QAM_Pareto_Lp2_data.tex <==
\path [draw=color1, very thin]
(axis cs:1.05346666666667,0)
--(axis cs:1.05346666666667,29.5833689618489)
--(axis cs:1.0602,29.5833689618489)
--(axis cs:1.0602,29.7908489927429)
--(axis cs:1.08173333333333,29.7908489927429)
--(axis cs:1.08173333333333,29.9276358042911)
--(axis cs:1.0969,29.9276358042911)
--(axis cs:1.0969,30.1488631086572)
--(axis cs:1.1189,30.1488631086572)
--(axis cs:1.1189,30.4051547781787)
--(axis cs:1.14463333333333,30.4051547781787)
--(axis cs:1.14463333333333,30.7244081984512)
--(axis cs:1.1878,30.7244081984512)
--(axis cs:1.1878,31.0243779262877)
--(axis cs:1.25976666666667,31.0243779262877)
--(axis cs:1.25976666666667,31.2880385419957)
--(axis cs:1.3547,31.2880385419957)
--(axis cs:1.3547,31.6851962164384)
--(axis cs:1.50436666666667,31.6851962164384)
--(axis cs:1.50436666666667,31.9802379163871)
--(axis cs:1.72773333333333,31.9802379163871)
--(axis cs:1.72773333333333,32.2741867138536)
--(axis cs:2.071,32.2741867138536)
--(axis cs:2.071,32.4080018682445)
--(axis cs:2.071,32.4080018682445)
--(axis cs:2.071,32.4080018682445)
--(axis cs:4.071,32.4080018682445)
--(axis cs:4.071,32.4080018682445)
--(axis cs:4.071,32.4080018682445)
--(axis cs:4.071,0);
\path [draw=color1, fill=color1, opacity=0.1, very thin]
(axis cs:1.05346666666667,0)
--(axis cs:1.05346666666667,29.5833689618489)
--(axis cs:1.0602,29.5833689618489)
--(axis cs:1.0602,29.7908489927429)
--(axis cs:1.08173333333333,29.7908489927429)
--(axis cs:1.08173333333333,29.9276358042911)
--(axis cs:1.0969,29.9276358042911)
--(axis cs:1.0969,30.1488631086572)
--(axis cs:1.1189,30.1488631086572)
--(axis cs:1.1189,30.4051547781787)
--(axis cs:1.14463333333333,30.4051547781787)
--(axis cs:1.14463333333333,30.7244081984512)
--(axis cs:1.1878,30.7244081984512)
--(axis cs:1.1878,31.0243779262877)
--(axis cs:1.25976666666667,31.0243779262877)
--(axis cs:1.25976666666667,31.2880385419957)
--(axis cs:1.3547,31.2880385419957)
--(axis cs:1.3547,31.6851962164384)
--(axis cs:1.50436666666667,31.6851962164384)
--(axis cs:1.50436666666667,31.9802379163871)
--(axis cs:1.72773333333333,31.9802379163871)
--(axis cs:1.72773333333333,32.2741867138536)
--(axis cs:2.071,32.2741867138536)
--(axis cs:2.071,32.4080018682445)
--(axis cs:2.071,32.4080018682445)
--(axis cs:2.071,32.4080018682445)
--(axis cs:4.071,32.4080018682445)
--(axis cs:4.071,32.4080018682445)
--(axis cs:4.071,0)
--(axis cs:4.071,0)
--(axis cs:4.071,0)
--(axis cs:2.071,0)
--(axis cs:2.071,0)
--(axis cs:2.071,0)
--(axis cs:2.071,0)
--(axis cs:1.72773333333333,0)
--(axis cs:1.72773333333333,0)
--(axis cs:1.50436666666667,0)
--(axis cs:1.50436666666667,0)
--(axis cs:1.3547,0)
--(axis cs:1.3547,0)
--(axis cs:1.25976666666667,0)
--(axis cs:1.25976666666667,0)
--(axis cs:1.1878,0)
--(axis cs:1.1878,0)
--(axis cs:1.14463333333333,0)
--(axis cs:1.14463333333333,0)
--(axis cs:1.1189,0)
--(axis cs:1.1189,0)
--(axis cs:1.0969,0)
--(axis cs:1.0969,0)
--(axis cs:1.08173333333333,0)
--(axis cs:1.08173333333333,0)
--(axis cs:1.0602,0)
--(axis cs:1.0602,0)
--(axis cs:1.05346666666667,0)
--cycle;


\path [draw=color2, very thin]
(axis cs:1.02033333333333,0)
--(axis cs:1.02033333333333,29.1283322711284)
--(axis cs:1.0459,29.1283322711284)
--(axis cs:1.0459,29.8376378136064)
--(axis cs:1.08046666666667,29.8376378136064)
--(axis cs:1.08046666666667,30.544213638549)
--(axis cs:1.1284,30.544213638549)
--(axis cs:1.1284,31.2317294872428)
--(axis cs:1.19126666666667,31.2317294872428)
--(axis cs:1.19126666666667,31.9013555622555)
--(axis cs:1.41623333333333,31.9013555622555)
--(axis cs:1.41623333333333,32.4264814462565)
--(axis cs:1.59433333333333,32.4264814462565)
--(axis cs:1.59433333333333,32.8141827475656)
--(axis cs:1.82656666666667,32.8141827475656)
--(axis cs:1.82656666666667,32.9974866503363)
--(axis cs:2.09896666666667,32.9974866503363)
--(axis cs:2.09896666666667,33.0032692964983)
--(axis cs:2.09896666666667,33.0032692964983)
--(axis cs:2.09896666666667,33.0032692964983)
--(axis cs:4.09896666666667,33.0032692964983)
--(axis cs:4.09896666666667,33.0032692964983)
--(axis cs:4.09896666666667,33.0032692964983)
--(axis cs:4.09896666666667,0);

\path [draw=color2, fill=color2, opacity=0.1, very thin]
(axis cs:1.02033333333333,0)
--(axis cs:1.02033333333333,29.1283322711284)
--(axis cs:1.0459,29.1283322711284)
--(axis cs:1.0459,29.8376378136064)
--(axis cs:1.08046666666667,29.8376378136064)
--(axis cs:1.08046666666667,30.544213638549)
--(axis cs:1.1284,30.544213638549)
--(axis cs:1.1284,31.2317294872428)
--(axis cs:1.19126666666667,31.2317294872428)
--(axis cs:1.19126666666667,31.9013555622555)
--(axis cs:1.41623333333333,31.9013555622555)
--(axis cs:1.41623333333333,32.4264814462565)
--(axis cs:1.59433333333333,32.4264814462565)
--(axis cs:1.59433333333333,32.8141827475656)
--(axis cs:1.82656666666667,32.8141827475656)
--(axis cs:1.82656666666667,32.9974866503363)
--(axis cs:2.09896666666667,32.9974866503363)
--(axis cs:2.09896666666667,33.0032692964983)
--(axis cs:2.09896666666667,33.0032692964983)
--(axis cs:2.09896666666667,33.0032692964983)
--(axis cs:4.09896666666667,33.0032692964983)
--(axis cs:4.09896666666667,33.0032692964983)
--(axis cs:4.09896666666667,0)
--(axis cs:4.09896666666667,0)
--(axis cs:4.09896666666667,0)
--(axis cs:2.09896666666667,0)
--(axis cs:2.09896666666667,0)
--(axis cs:2.09896666666667,0)
--(axis cs:2.09896666666667,0)
--(axis cs:1.82656666666667,0)
--(axis cs:1.82656666666667,0)
--(axis cs:1.59433333333333,0)
--(axis cs:1.59433333333333,0)
--(axis cs:1.41623333333333,0)
--(axis cs:1.41623333333333,0)
--(axis cs:1.19126666666667,0)
--(axis cs:1.19126666666667,0)
--(axis cs:1.1284,0)
--(axis cs:1.1284,0)
--(axis cs:1.08046666666667,0)
--(axis cs:1.08046666666667,0)
--(axis cs:1.0459,0)
--(axis cs:1.0459,0)
--(axis cs:1.02033333333333,0)
--cycle;

\path [draw=color3, very thin]
(axis cs:1.02323333333333,0)
--(axis cs:1.02323333333333,29.2799050722285)
--(axis cs:1.04853333333333,29.2799050722285)
--(axis cs:1.04853333333333,30.0018780551232)
--(axis cs:1.07906666666667,30.0018780551232)
--(axis cs:1.07906666666667,30.7476679209923)
--(axis cs:1.1356,30.7476679209923)
--(axis cs:1.1356,31.4034600569897)
--(axis cs:1.20583333333333,31.4034600569897)
--(axis cs:1.20583333333333,32.0406113665479)
--(axis cs:1.43636666666667,32.0406113665479)
--(axis cs:1.43636666666667,32.6160655897613)
--(axis cs:1.6342,32.6160655897613)
--(axis cs:1.6342,32.9773630795761)
--(axis cs:1.88833333333333,32.9773630795761)
--(axis cs:1.88833333333333,33.1068510177601)
--(axis cs:1.88833333333333,33.1068510177601)
--(axis cs:1.88833333333333,33.1068510177601)
--(axis cs:3.88833333333333,33.1068510177601)
--(axis cs:3.88833333333333,33.1068510177601)
--(axis cs:3.88833333333333,33.1068510177601)
--(axis cs:3.88833333333333,0);

\path [draw=color3, fill=color3, opacity=0.1, very thin]
(axis cs:1.02323333333333,0)
--(axis cs:1.02323333333333,29.2799050722285)
--(axis cs:1.04853333333333,29.2799050722285)
--(axis cs:1.04853333333333,30.0018780551232)
--(axis cs:1.07906666666667,30.0018780551232)
--(axis cs:1.07906666666667,30.7476679209923)
--(axis cs:1.1356,30.7476679209923)
--(axis cs:1.1356,31.4034600569897)
--(axis cs:1.20583333333333,31.4034600569897)
--(axis cs:1.20583333333333,32.0406113665479)
--(axis cs:1.43636666666667,32.0406113665479)
--(axis cs:1.43636666666667,32.6160655897613)
--(axis cs:1.6342,32.6160655897613)
--(axis cs:1.6342,32.9773630795761)
--(axis cs:1.88833333333333,32.9773630795761)
--(axis cs:1.88833333333333,33.1068510177601)
--(axis cs:1.88833333333333,33.1068510177601)
--(axis cs:1.88833333333333,33.1068510177601)
--(axis cs:3.88833333333333,33.1068510177601)
--(axis cs:3.88833333333333,33.1068510177601)
--(axis cs:3.88833333333333,0)
--(axis cs:3.88833333333333,0)
--(axis cs:3.88833333333333,0)
--(axis cs:1.88833333333333,0)
--(axis cs:1.88833333333333,0)
--(axis cs:1.88833333333333,0)
--(axis cs:1.88833333333333,0)
--(axis cs:1.6342,0)
--(axis cs:1.6342,0)
--(axis cs:1.43636666666667,0)
--(axis cs:1.43636666666667,0)
--(axis cs:1.20583333333333,0)
--(axis cs:1.20583333333333,0)
--(axis cs:1.1356,0)
--(axis cs:1.1356,0)
--(axis cs:1.07906666666667,0)
--(axis cs:1.07906666666667,0)
--(axis cs:1.04853333333333,0)
--(axis cs:1.04853333333333,0)
--(axis cs:1.02323333333333,0)
--cycle;

\path [draw=color4, very thin]
(axis cs:8.03683333333333,0)
--(axis cs:8.03683333333333,25.0202080865717)
--(axis cs:1.0659,25.0202080865717)
--(axis cs:1.0659,29.7641426734502)
--(axis cs:1.07476666666667,29.7641426734502)
--(axis cs:1.07476666666667,29.9477338704258)
--(axis cs:1.0987,29.9477338704258)
--(axis cs:1.0987,30.0995427542489)
--(axis cs:1.11123333333333,30.0995427542489)
--(axis cs:1.11123333333333,30.3148665832052)
--(axis cs:1.1398,30.3148665832052)
--(axis cs:1.1398,30.5731455766785)
--(axis cs:1.1717,30.5731455766785)
--(axis cs:1.1717,30.8270609940054)
--(axis cs:1.21303333333333,30.8270609940054)
--(axis cs:1.21303333333333,31.1750157855428)
--(axis cs:1.2824,31.1750157855428)
--(axis cs:1.2824,31.4700611197269)
--(axis cs:1.37866666666667,31.4700611197269)
--(axis cs:1.37866666666667,31.8419742807317)
--(axis cs:1.5494,31.8419742807317)
--(axis cs:1.5494,32.1783383229438)
--(axis cs:1.79846666666667,32.1783383229438)
--(axis cs:1.79846666666667,32.442122012211)
--(axis cs:2.17126666666667,32.442122012211)
--(axis cs:2.17126666666667,32.506061067722)
--(axis cs:2.17126666666667,32.506061067722)
--(axis cs:2.17126666666667,32.506061067722)
--(axis cs:12.1712666666667,32.506061067722)
--(axis cs:12.1712666666667,32.506061067722)
--(axis cs:12.1712666666667,32.506061067722)
--(axis cs:12.1712666666667,0);
\path [draw=color4, fill=color4, opacity=0.1, very thin]
(axis cs:8.03683333333333,0)
--(axis cs:8.03683333333333,25.0202080865717)
--(axis cs:1.0659,25.0202080865717)
--(axis cs:1.0659,29.7641426734502)
--(axis cs:1.07476666666667,29.7641426734502)
--(axis cs:1.07476666666667,29.9477338704258)
--(axis cs:1.0987,29.9477338704258)
--(axis cs:1.0987,30.0995427542489)
--(axis cs:1.11123333333333,30.0995427542489)
--(axis cs:1.11123333333333,30.3148665832052)
--(axis cs:1.1398,30.3148665832052)
--(axis cs:1.1398,30.5731455766785)
--(axis cs:1.1717,30.5731455766785)
--(axis cs:1.1717,30.8270609940054)
--(axis cs:1.21303333333333,30.8270609940054)
--(axis cs:1.21303333333333,31.1750157855428)
--(axis cs:1.2824,31.1750157855428)
--(axis cs:1.2824,31.4700611197269)
--(axis cs:1.37866666666667,31.4700611197269)
--(axis cs:1.37866666666667,31.8419742807317)
--(axis cs:1.5494,31.8419742807317)
--(axis cs:1.5494,32.1783383229438)
--(axis cs:1.79846666666667,32.1783383229438)
--(axis cs:1.79846666666667,32.442122012211)
--(axis cs:2.17126666666667,32.442122012211)
--(axis cs:2.17126666666667,32.506061067722)
--(axis cs:2.17126666666667,32.506061067722)
--(axis cs:2.17126666666667,32.506061067722)
--(axis cs:12.1712666666667,32.506061067722)
--(axis cs:12.1712666666667,32.506061067722)
--(axis cs:12.1712666666667,0)
--(axis cs:12.1712666666667,0)
--(axis cs:12.1712666666667,0)
--(axis cs:2.17126666666667,0)
--(axis cs:2.17126666666667,0)
--(axis cs:2.17126666666667,0)
--(axis cs:2.17126666666667,0)
--(axis cs:1.79846666666667,0)
--(axis cs:1.79846666666667,0)
--(axis cs:1.5494,0)
--(axis cs:1.5494,0)
--(axis cs:1.37866666666667,0)
--(axis cs:1.37866666666667,0)
--(axis cs:1.2824,0)
--(axis cs:1.2824,0)
--(axis cs:1.21303333333333,0)
--(axis cs:1.21303333333333,0)
--(axis cs:1.1717,0)
--(axis cs:1.1717,0)
--(axis cs:1.1398,0)
--(axis cs:1.1398,0)
--(axis cs:1.11123333333333,0)
--(axis cs:1.11123333333333,0)
--(axis cs:1.0987,0)
--(axis cs:1.0987,0)
--(axis cs:1.07476666666667,0)
--(axis cs:1.07476666666667,0)
--(axis cs:1.0659,0)
--(axis cs:1.0659,0)
--(axis cs:8.03683333333333,0)
--cycle;

\addplot [semithick, color6, mark=diamond*, mark size=3, mark options={solid}, only marks]
table {%
1.2043 32.2797181925773
1.343667 32.7541056734799
1.242933 32.4400856281369
1.290133 32.5872243156608
1.305767 32.5043902742771
1.310367 32.7446129954272
1.506033 33.002188615784
1.603033 33.1549943336571
1.654233 33.2201478922324
};

\addplot [semithick, color5, mark=diamond*, mark size=3, mark options={solid}, only marks]
table {%
1.120667 31.5525111976623
1.123733 31.5980988191451
1.161 31.9104594561253
1.1498 31.8742812148474
1.1448 31.6396378122303
1.1589 31.8928965300749
1.244367 32.3049754240405
1.259633 32.4670116743245
1.442333 32.9902506482745
};


==> tikzplotlib_figs_icmlcn/Fading_test_Pareto_Lp1_data.tex <==
\path [draw=color1, very thin]
(axis cs:1.6253,0)
--(axis cs:1.6253,30.777083930614)
--(axis cs:1.6594,30.777083930614)
--(axis cs:1.6594,31.0330862470114)
--(axis cs:1.72243333333333,31.0330862470114)
--(axis cs:1.72243333333333,31.2069768538309)
--(axis cs:1.8176,31.2069768538309)
--(axis cs:1.8176,31.2812259838063)
--(axis cs:1.88896666666667,31.2812259838063)
--(axis cs:1.88896666666667,31.7190484154324)
--(axis cs:2.00616666666667,31.7190484154324)
--(axis cs:2.00616666666667,31.8356283807124)
--(axis cs:2.13256666666667,31.8356283807124)
--(axis cs:2.13256666666667,31.9951077240732)
--(axis cs:2.3012,31.9951077240732)
--(axis cs:2.3012,32.1622682407445)
--(axis cs:2.46553333333333,32.1622682407445)
--(axis cs:2.46553333333333,32.509428798634)
--(axis cs:3.03883333333333,32.509428798634)
--(axis cs:3.03883333333333,32.576530887531)
--(axis cs:3.34563333333333,32.576530887531)
--(axis cs:3.34563333333333,32.6453126828412)
--(axis cs:3.75586666666667,32.6453126828412)
--(axis cs:3.75586666666667,32.6914043029019)
--(axis cs:3.75586666666667,32.6914043029019)
--(axis cs:3.75586666666667,32.6914043029019)
--(axis cs:13.7558666666667,32.6914043029019)
--(axis cs:13.7558666666667,32.6914043029019)
--(axis cs:13.7558666666667,32.6914043029019)
--(axis cs:13.7558666666667,0);

\path [draw=color1, fill=color1, opacity=0.1, very thin]
(axis cs:1.6253,0)
--(axis cs:1.6253,30.777083930614)
--(axis cs:1.6594,30.777083930614)
--(axis cs:1.6594,31.0330862470114)
--(axis cs:1.72243333333333,31.0330862470114)
--(axis cs:1.72243333333333,31.2069768538309)
--(axis cs:1.8176,31.2069768538309)
--(axis cs:1.8176,31.2812259838063)
--(axis cs:1.88896666666667,31.2812259838063)
--(axis cs:1.88896666666667,31.7190484154324)
--(axis cs:2.00616666666667,31.7190484154324)
--(axis cs:2.00616666666667,31.8356283807124)
--(axis cs:2.13256666666667,31.8356283807124)
--(axis cs:2.13256666666667,31.9951077240732)
--(axis cs:2.3012,31.9951077240732)
--(axis cs:2.3012,32.1622682407445)
--(axis cs:2.46553333333333,32.1622682407445)
--(axis cs:2.46553333333333,32.509428798634)
--(axis cs:3.03883333333333,32.509428798634)
--(axis cs:3.03883333333333,32.576530887531)
--(axis cs:3.34563333333333,32.576530887531)
--(axis cs:3.34563333333333,32.6453126828412)
--(axis cs:3.75586666666667,32.6453126828412)
--(axis cs:3.75586666666667,32.6914043029019)
--(axis cs:3.75586666666667,32.6914043029019)
--(axis cs:3.75586666666667,32.6914043029019)
--(axis cs:13.7558666666667,32.6914043029019)
--(axis cs:13.7558666666667,32.6914043029019)
--(axis cs:13.7558666666667,0)
--(axis cs:13.7558666666667,0)
--(axis cs:13.7558666666667,0)
--(axis cs:3.75586666666667,0)
--(axis cs:3.75586666666667,0)
--(axis cs:3.75586666666667,0)
--(axis cs:3.75586666666667,0)
--(axis cs:3.34563333333333,0)
--(axis cs:3.34563333333333,0)
--(axis cs:3.03883333333333,0)
--(axis cs:3.03883333333333,0)
--(axis cs:2.46553333333333,0)
--(axis cs:2.46553333333333,0)
--(axis cs:2.3012,0)
--(axis cs:2.3012,0)
--(axis cs:2.13256666666667,0)
--(axis cs:2.13256666666667,0)
--(axis cs:2.00616666666667,0)
--(axis cs:2.00616666666667,0)
--(axis cs:1.88896666666667,0)
--(axis cs:1.88896666666667,0)
--(axis cs:1.8176,0)
--(axis cs:1.8176,0)
--(axis cs:1.72243333333333,0)
--(axis cs:1.72243333333333,0)
--(axis cs:1.6594,0)
--(axis cs:1.6594,0)
--(axis cs:1.6253,0)
--cycle;

\path [draw=color2, very thin]
(axis cs:2.0741,0)
--(axis cs:2.0741,30.4354863584825)
--(axis cs:2.14936666666667,30.4354863584825)
--(axis cs:2.14936666666667,30.8846187797072)
--(axis cs:2.25916666666667,30.8846187797072)
--(axis cs:2.25916666666667,31.1472917148092)
--(axis cs:2.33473333333333,31.1472917148092)
--(axis cs:2.33473333333333,31.6251195115726)
--(axis cs:2.46083333333333,31.6251195115726)
--(axis cs:2.46083333333333,31.9131337390274)
--(axis cs:4.0917,31.9131337390274)
--(axis cs:4.0917,31.913692271492)
--(axis cs:4.0917,31.913692271492)
--(axis cs:4.0917,31.913692271492)
--(axis cs:14.0917,31.913692271492)
--(axis cs:14.0917,31.913692271492)
--(axis cs:14.0917,31.913692271492)
--(axis cs:14.0917,0);

\path [draw=color2, fill=color2, opacity=0.1, very thin]
(axis cs:2.0741,0)
--(axis cs:2.0741,30.4354863584825)
--(axis cs:2.14936666666667,30.4354863584825)
--(axis cs:2.14936666666667,30.8846187797072)
--(axis cs:2.25916666666667,30.8846187797072)
--(axis cs:2.25916666666667,31.1472917148092)
--(axis cs:2.33473333333333,31.1472917148092)
--(axis cs:2.33473333333333,31.6251195115726)
--(axis cs:2.46083333333333,31.6251195115726)
--(axis cs:2.46083333333333,31.9131337390274)
--(axis cs:4.0917,31.9131337390274)
--(axis cs:4.0917,31.913692271492)
--(axis cs:4.0917,31.913692271492)
--(axis cs:4.0917,31.913692271492)
--(axis cs:14.0917,31.913692271492)
--(axis cs:14.0917,31.913692271492)
--(axis cs:14.0917,0)
--(axis cs:14.0917,0)
--(axis cs:14.0917,0)
--(axis cs:4.0917,0)
--(axis cs:4.0917,0)
--(axis cs:4.0917,0)
--(axis cs:4.0917,0)
--(axis cs:2.46083333333333,0)
--(axis cs:2.46083333333333,0)
--(axis cs:2.33473333333333,0)
--(axis cs:2.33473333333333,0)
--(axis cs:2.25916666666667,0)
--(axis cs:2.25916666666667,0)
--(axis cs:2.14936666666667,0)
--(axis cs:2.14936666666667,0)
--(axis cs:2.0741,0)
--cycle;

\path [draw=color3, very thin]
(axis cs:2.1002,0)
--(axis cs:2.1002,30.5627241008485)
--(axis cs:2.20403333333333,30.5627241008485)
--(axis cs:2.20403333333333,30.9065242864559)
--(axis cs:2.30016666666667,30.9065242864559)
--(axis cs:2.30016666666667,31.3096416085753)
--(axis cs:2.43113333333333,31.3096416085753)
--(axis cs:2.43113333333333,31.6053785161232)
--(axis cs:2.54543333333333,31.6053785161232)
--(axis cs:2.54543333333333,32.0419375880382)
--(axis cs:2.54543333333333,32.0419375880382)
--(axis cs:2.54543333333333,32.0419375880382)
--(axis cs:12.5454333333333,32.0419375880382)
--(axis cs:12.5454333333333,32.0419375880382)
--(axis cs:12.5454333333333,32.0419375880382)
--(axis cs:12.5454333333333,0);
\path [draw=color3, fill=color3, opacity=0.1, very thin]
(axis cs:2.1002,0)
--(axis cs:2.1002,30.5627241008485)
--(axis cs:2.20403333333333,30.5627241008485)
--(axis cs:2.20403333333333,30.9065242864559)
--(axis cs:2.30016666666667,30.9065242864559)
--(axis cs:2.30016666666667,31.3096416085753)
--(axis cs:2.43113333333333,31.3096416085753)
--(axis cs:2.43113333333333,31.6053785161232)
--(axis cs:2.54543333333333,31.6053785161232)
--(axis cs:2.54543333333333,32.0419375880382)
--(axis cs:2.54543333333333,32.0419375880382)
--(axis cs:2.54543333333333,32.0419375880382)
--(axis cs:12.5454333333333,32.0419375880382)
--(axis cs:12.5454333333333,32.0419375880382)
--(axis cs:12.5454333333333,0)
--(axis cs:12.5454333333333,0)
--(axis cs:12.5454333333333,0)
--(axis cs:2.54543333333333,0)
--(axis cs:2.54543333333333,0)
--(axis cs:2.54543333333333,0)
--(axis cs:2.54543333333333,0)
--(axis cs:2.43113333333333,0)
--(axis cs:2.43113333333333,0)
--(axis cs:2.30016666666667,0)
--(axis cs:2.30016666666667,0)
--(axis cs:2.20403333333333,0)
--(axis cs:2.20403333333333,0)
--(axis cs:2.1002,0)
--cycle;

\path [draw=color4, very thin]
(axis cs:1.68513333333333,0)
--(axis cs:1.68513333333333,30.577679595808)
--(axis cs:1.68513333333333,30.9644899727598)
--(axis cs:1.73166666666667,30.9644899727598)
--(axis cs:1.73166666666667,31.0509434361363)
--(axis cs:1.7762,31.0509434361363)
--(axis cs:1.7762,31.3525708791972)
--(axis cs:1.87336666666667,31.3525708791972)
--(axis cs:1.87336666666667,31.5023168985464)
--(axis cs:1.9284,31.5023168985464)
--(axis cs:1.9284,31.8617351492612)
--(axis cs:2.0715,31.8617351492612)
--(axis cs:2.0715,31.9062833797655)
--(axis cs:2.21046666666667,31.9062833797655)
--(axis cs:2.21046666666667,32.1328309665875)
--(axis cs:2.38876666666667,32.1328309665875)
--(axis cs:2.38876666666667,32.4020955458521)
--(axis cs:2.5565,32.4020955458521)
--(axis cs:2.5565,32.5155856316447)
--(axis cs:2.80933333333333,32.5155856316447)
--(axis cs:2.80933333333333,32.8362442050687)
--(axis cs:3.0765,32.8362442050687)
--(axis cs:3.0765,32.9359092633067)
--(axis cs:3.41836666666667,32.9359092633067)
--(axis cs:3.41836666666667,33.1628840727983)
--(axis cs:3.41836666666667,33.1628840727983)
--(axis cs:3.41836666666667,33.1628840727983)
--(axis cs:13.4183666666667,33.1628840727983)
--(axis cs:13.4183666666667,33.1628840727983)
--(axis cs:13.4183666666667,33.1628840727983)
--(axis cs:13.4183666666667,0);
\path [draw=color4, fill=color4, opacity=0.1, very thin]
(axis cs:1.68513333333333,0)
--(axis cs:1.68513333333333,30.577679595808)
--(axis cs:1.68513333333333,30.9644899727598)
--(axis cs:1.73166666666667,30.9644899727598)
--(axis cs:1.73166666666667,31.0509434361363)
--(axis cs:1.7762,31.0509434361363)
--(axis cs:1.7762,31.3525708791972)
--(axis cs:1.87336666666667,31.3525708791972)
--(axis cs:1.87336666666667,31.5023168985464)
--(axis cs:1.9284,31.5023168985464)
--(axis cs:1.9284,31.8617351492612)
--(axis cs:2.0715,31.8617351492612)
--(axis cs:2.0715,31.9062833797655)
--(axis cs:2.21046666666667,31.9062833797655)
--(axis cs:2.21046666666667,32.1328309665875)
--(axis cs:2.38876666666667,32.1328309665875)
--(axis cs:2.38876666666667,32.4020955458521)
--(axis cs:2.5565,32.4020955458521)
--(axis cs:2.5565,32.5155856316447)
--(axis cs:2.80933333333333,32.5155856316447)
--(axis cs:2.80933333333333,32.8362442050687)
--(axis cs:3.0765,32.8362442050687)
--(axis cs:3.0765,32.9359092633067)
--(axis cs:3.41836666666667,32.9359092633067)
--(axis cs:3.41836666666667,33.1628840727983)
--(axis cs:3.41836666666667,33.1628840727983)
--(axis cs:3.41836666666667,33.1628840727983)
--(axis cs:13.4183666666667,33.1628840727983)
--(axis cs:13.4183666666667,33.1628840727983)
--(axis cs:13.4183666666667,0)
--(axis cs:13.4183666666667,0)
--(axis cs:13.4183666666667,0)
--(axis cs:3.41836666666667,0)
--(axis cs:3.41836666666667,0)
--(axis cs:3.41836666666667,0)
--(axis cs:3.41836666666667,0)
--(axis cs:3.0765,0)
--(axis cs:3.0765,0)
--(axis cs:2.80933333333333,0)
--(axis cs:2.80933333333333,0)
--(axis cs:2.5565,0)
--(axis cs:2.5565,0)
--(axis cs:2.38876666666667,0)
--(axis cs:2.38876666666667,0)
--(axis cs:2.21046666666667,0)
--(axis cs:2.21046666666667,0)
--(axis cs:2.0715,0)
--(axis cs:2.0715,0)
--(axis cs:1.9284,0)
--(axis cs:1.9284,0)
--(axis cs:1.87336666666667,0)
--(axis cs:1.87336666666667,0)
--(axis cs:1.7762,0)
--(axis cs:1.7762,0)
--(axis cs:1.73166666666667,0)
--(axis cs:1.73166666666667,0)
--(axis cs:1.68513333333333,0)
--(axis cs:1.68513333333333,0)
--(axis cs:8.52373333333333,0)
--cycle;

\addplot [semithick, color6, mark=diamond*, mark size=3, mark options={solid}, only marks]
table {%
2.2151 33.3448001413927
2.1389 33.3220326253688
2.237 33.4188667820006
2.46866666666667 33.3522514495984
2.7121 33.2014742370229
2.39966666666667 33.4105503030611
2.62246666666667 33.6973092368919
2.68516666666667 33.5638720580968
3.80846666666667 32.7862149214946
};

\addplot [semithick, color5, mark=diamond*, mark size=3, mark options={solid}, only marks]
table {%
1.7161 32.4101822636796
1.7551 32.4760024388848
1.74086666666667 32.4284226467915
1.84046666666667 32.6875322586594
1.89846666666667 32.8048512510924
1.9322 33.0103884369764
2.0389 33.1127376321725
2.09856666666667 33.16904515207
2.4729 33.2050171206216
};

==> tikzplotlib_figs_icmlcn/Fading_test_Pareto_Lp2_data.tex <==
\path [draw=color1, very thin]
(axis cs:1.6253,0)
--(axis cs:1.6253,28.6089225255825)
--(axis cs:1.6594,28.6089225255825)
--(axis cs:1.6594,28.8097203729911)
--(axis cs:1.72243333333333,28.8097203729911)
--(axis cs:1.72243333333333,28.9235910623095)
--(axis cs:1.8176,28.9235910623095)
--(axis cs:1.8176,28.9365494666052)
--(axis cs:1.88896666666667,28.9365494666052)
--(axis cs:1.88896666666667,29.2796078805151)
--(axis cs:2.00616666666667,29.2796078805151)
--(axis cs:2.00616666666667,29.3097656375673)
--(axis cs:2.13256666666667,29.3097656375673)
--(axis cs:2.13256666666667,29.3865946692021)
--(axis cs:2.3012,29.3865946692021)
--(axis cs:2.3012,29.4345401690346)
--(axis cs:2.46553333333333,29.4345401690346)
--(axis cs:2.46553333333333,29.6467582533085)
--(axis cs:2.46553333333333,29.6467582533085)
--(axis cs:2.46553333333333,29.6467582533085)
--(axis cs:12.4655333333333,29.6467582533085)
--(axis cs:12.4655333333333,29.6467582533085)
--(axis cs:12.4655333333333,29.6467582533085)
--(axis cs:12.4655333333333,0);

\path [draw=color1, fill=color1, opacity=0.1, very thin]
(axis cs:1.6253,0)
--(axis cs:1.6253,28.6089225255825)
--(axis cs:1.6594,28.6089225255825)
--(axis cs:1.6594,28.8097203729911)
--(axis cs:1.72243333333333,28.8097203729911)
--(axis cs:1.72243333333333,28.9235910623095)
--(axis cs:1.8176,28.9235910623095)
--(axis cs:1.8176,28.9365494666052)
--(axis cs:1.88896666666667,28.9365494666052)
--(axis cs:1.88896666666667,29.2796078805151)
--(axis cs:2.00616666666667,29.2796078805151)
--(axis cs:2.00616666666667,29.3097656375673)
--(axis cs:2.13256666666667,29.3097656375673)
--(axis cs:2.13256666666667,29.3865946692021)
--(axis cs:2.3012,29.3865946692021)
--(axis cs:2.3012,29.4345401690346)
--(axis cs:2.46553333333333,29.4345401690346)
--(axis cs:2.46553333333333,29.6467582533085)
--(axis cs:2.46553333333333,29.6467582533085)
--(axis cs:2.46553333333333,29.6467582533085)
--(axis cs:12.4655333333333,29.6467582533085)
--(axis cs:12.4655333333333,29.6467582533085)
--(axis cs:12.4655333333333,0)
--(axis cs:12.4655333333333,0)
--(axis cs:12.4655333333333,0)
--(axis cs:2.46553333333333,0)
--(axis cs:2.46553333333333,0)
--(axis cs:2.46553333333333,0)
--(axis cs:2.46553333333333,0)
--(axis cs:2.3012,0)
--(axis cs:2.3012,0)
--(axis cs:2.13256666666667,0)
--(axis cs:2.13256666666667,0)
--(axis cs:2.00616666666667,0)
--(axis cs:2.00616666666667,0)
--(axis cs:1.88896666666667,0)
--(axis cs:1.88896666666667,0)
--(axis cs:1.8176,0)
--(axis cs:1.8176,0)
--(axis cs:1.72243333333333,0)
--(axis cs:1.72243333333333,0)
--(axis cs:1.6594,0)
--(axis cs:1.6594,0)
--(axis cs:1.6253,0)
--cycle;

\path [draw=color2, very thin]
(axis cs:2.0741,0)
--(axis cs:2.0741,28.2258680468521)
--(axis cs:2.14936666666667,28.2258680468521)
--(axis cs:2.14936666666667,28.5765517153333)
--(axis cs:2.25916666666667,28.5765517153333)
--(axis cs:2.25916666666667,28.7402306096226)
--(axis cs:2.33473333333333,28.7402306096226)
--(axis cs:2.33473333333333,29.1054137617776)
--(axis cs:2.46083333333333,29.1054137617776)
--(axis cs:2.46083333333333,29.2791276259454)
--(axis cs:2.46083333333333,29.2791276259454)
--(axis cs:2.46083333333333,29.2791276259454)
--(axis cs:12.4608333333333,29.2791276259454)
--(axis cs:12.4608333333333,29.2791276259454)
--(axis cs:12.4608333333333,29.2791276259454)
--(axis cs:12.4608333333333,0);

\path [draw=color2, fill=color2, opacity=0.1, very thin]
(axis cs:2.0741,0)
--(axis cs:2.0741,28.2258680468521)
--(axis cs:2.14936666666667,28.2258680468521)
--(axis cs:2.14936666666667,28.5765517153333)
--(axis cs:2.25916666666667,28.5765517153333)
--(axis cs:2.25916666666667,28.7402306096226)
--(axis cs:2.33473333333333,28.7402306096226)
--(axis cs:2.33473333333333,29.1054137617776)
--(axis cs:2.46083333333333,29.1054137617776)
--(axis cs:2.46083333333333,29.2791276259454)
--(axis cs:2.46083333333333,29.2791276259454)
--(axis cs:2.46083333333333,29.2791276259454)
--(axis cs:12.4608333333333,29.2791276259454)
--(axis cs:12.4608333333333,29.2791276259454)
--(axis cs:12.4608333333333,0)
--(axis cs:12.4608333333333,0)
--(axis cs:12.4608333333333,0)
--(axis cs:2.46083333333333,0)
--(axis cs:2.46083333333333,0)
--(axis cs:2.46083333333333,0)
--(axis cs:2.46083333333333,0)
--(axis cs:2.33473333333333,0)
--(axis cs:2.33473333333333,0)
--(axis cs:2.25916666666667,0)
--(axis cs:2.25916666666667,0)
--(axis cs:2.14936666666667,0)
--(axis cs:2.14936666666667,0)
--(axis cs:2.0741,0)
--cycle;

\path [draw=color3, very thin]
(axis cs:2.1002,0)
--(axis cs:2.1002,28.3293612493651)
--(axis cs:2.20403333333333,28.3293612493651)
--(axis cs:2.20403333333333,28.5738913412465)
--(axis cs:2.30016666666667,28.5738913412465)
--(axis cs:2.30016666666667,28.8708513101713)
--(axis cs:2.43113333333333,28.8708513101713)
--(axis cs:2.43113333333333,29.0576385442336)
--(axis cs:2.54543333333333,29.0576385442336)
--(axis cs:2.54543333333333,29.3718878476196)
--(axis cs:2.54543333333333,29.3718878476196)
--(axis cs:2.54543333333333,29.3718878476196)
--(axis cs:12.5454333333333,29.3718878476196)
--(axis cs:12.5454333333333,29.3718878476196)
--(axis cs:12.5454333333333,29.3718878476196)
--(axis cs:12.5454333333333,0);
\path [draw=color3, fill=color3, opacity=0.1, very thin]
(axis cs:2.1002,0)
--(axis cs:2.1002,28.3293612493651)
--(axis cs:2.20403333333333,28.3293612493651)
--(axis cs:2.20403333333333,28.5738913412465)
--(axis cs:2.30016666666667,28.5738913412465)
--(axis cs:2.30016666666667,28.8708513101713)
--(axis cs:2.43113333333333,28.8708513101713)
--(axis cs:2.43113333333333,29.0576385442336)
--(axis cs:2.54543333333333,29.0576385442336)
--(axis cs:2.54543333333333,29.3718878476196)
--(axis cs:2.54543333333333,29.3718878476196)
--(axis cs:2.54543333333333,29.3718878476196)
--(axis cs:12.5454333333333,29.3718878476196)
--(axis cs:12.5454333333333,29.3718878476196)
--(axis cs:12.5454333333333,0)
--(axis cs:12.5454333333333,0)
--(axis cs:12.5454333333333,0)
--(axis cs:2.54543333333333,0)
--(axis cs:2.54543333333333,0)
--(axis cs:2.54543333333333,0)
--(axis cs:2.54543333333333,0)
--(axis cs:2.43113333333333,0)
--(axis cs:2.43113333333333,0)
--(axis cs:2.30016666666667,0)
--(axis cs:2.30016666666667,0)
--(axis cs:2.20403333333333,0)
--(axis cs:2.20403333333333,0)
--(axis cs:2.1002,0)
--cycle;


\path [draw=color4, very thin]
(axis cs:8.52373333333333,0)
--(axis cs:8.52373333333333,25.3297658043658)
--(axis cs:1.68513333333333,25.3297658043658)
--(axis cs:1.68513333333333,28.7506038289506)
--(axis cs:1.73166666666667,28.7506038289506)
--(axis cs:1.73166666666667,28.7887218014748)
--(axis cs:1.7762,28.7887218014748)
--(axis cs:1.7762,29.0295822702347)
--(axis cs:1.87336666666667,29.0295822702347)
--(axis cs:1.87336666666667,29.1056414483173)
--(axis cs:1.9284,29.1056414483173)
--(axis cs:1.9284,29.3892722122556)
--(axis cs:2.21046666666667,29.3892722122556)
--(axis cs:2.21046666666667,29.4612589563174)
--(axis cs:2.38876666666667,29.4612589563174)
--(axis cs:2.38876666666667,29.6074956990339)
--(axis cs:2.80933333333333,29.6074956990339)
--(axis cs:2.80933333333333,29.7549146531082)
--(axis cs:2.80933333333333,29.7549146531082)
--(axis cs:2.80933333333333,29.7549146531082)
--(axis cs:12.8093333333333,29.7549146531082)
--(axis cs:12.8093333333333,29.7549146531082)
--(axis cs:12.8093333333333,29.7549146531082)
--(axis cs:12.8093333333333,0);
\path [draw=color4, fill=color4, opacity=0.1, very thin]
(axis cs:8.52373333333333,0)
--(axis cs:8.52373333333333,25.3297658043658)
--(axis cs:1.68513333333333,25.3297658043658)
--(axis cs:1.68513333333333,28.7506038289506)
--(axis cs:1.73166666666667,28.7506038289506)
--(axis cs:1.73166666666667,28.7887218014748)
--(axis cs:1.7762,28.7887218014748)
--(axis cs:1.7762,29.0295822702347)
--(axis cs:1.87336666666667,29.0295822702347)
--(axis cs:1.87336666666667,29.1056414483173)
--(axis cs:1.9284,29.1056414483173)
--(axis cs:1.9284,29.3892722122556)
--(axis cs:2.21046666666667,29.3892722122556)
--(axis cs:2.21046666666667,29.4612589563174)
--(axis cs:2.38876666666667,29.4612589563174)
--(axis cs:2.38876666666667,29.6074956990339)
--(axis cs:2.80933333333333,29.6074956990339)
--(axis cs:2.80933333333333,29.7549146531082)
--(axis cs:2.80933333333333,29.7549146531082)
--(axis cs:2.80933333333333,29.7549146531082)
--(axis cs:12.8093333333333,29.7549146531082)
--(axis cs:12.8093333333333,29.7549146531082)
--(axis cs:12.8093333333333,0)
--(axis cs:12.8093333333333,0)
--(axis cs:12.8093333333333,0)
--(axis cs:2.80933333333333,0)
--(axis cs:2.80933333333333,0)
--(axis cs:2.80933333333333,0)
--(axis cs:2.80933333333333,0)
--(axis cs:2.38876666666667,0)
--(axis cs:2.38876666666667,0)
--(axis cs:2.21046666666667,0)
--(axis cs:2.21046666666667,0)
--(axis cs:1.9284,0)
--(axis cs:1.9284,0)
--(axis cs:1.87336666666667,0)
--(axis cs:1.87336666666667,0)
--(axis cs:1.7762,0)
--(axis cs:1.7762,0)
--(axis cs:1.73166666666667,0)
--(axis cs:1.73166666666667,0)
--(axis cs:1.68513333333333,0)
--(axis cs:1.68513333333333,0)
--(axis cs:8.52373333333333,0)
--cycle;

\addplot [semithick, color6, mark=diamond*, mark size=3, mark options={solid}, only marks]
table {%
1.69643333333333 29.9855607623728
1.8546 30.2333132881076
1.75913333333333 30.2910902472346
1.8106 30.2607017526675
1.82773333333333 30.2613583515523
1.83583333333333 30.0744705246329
2.01373333333333 30.4482862895368
2.12566666666667 30.5929152176926
4.6336 27.840428276654
};

\addplot [semithick, color5, mark=diamond*, mark size=3, mark options={solid}, only marks]
table {%
1.61096666666667 29.6337615457525
1.6144 29.6400668814103
1.61036666666667 29.6879176092706
1.6688 29.5965130807073
1.6291 29.6721615744372
1.68896666666667 29.7032042735874
1.77463333333333 29.7872399568002
1.8562 30.1879589917492
1.92536666666667 30.2984199286454
};

==> tikzplotlib_figs_icmlcn/QPSK_Pareto_Lp1_data.tex <==
\path [draw=color1, very thin]
(axis cs:1.0791,0)
--(axis cs:1.0791,7.99429013865697)
--(axis cs:1.08885,7.99429013865697)
--(axis cs:1.08885,8.02755847224052)
--(axis cs:1.10855,8.02755847224052)
--(axis cs:1.10855,8.05428863622945)
--(axis cs:1.1329,8.05428863622945)
--(axis cs:1.1329,8.10699471053411)
--(axis cs:1.15915,8.10699471053411)
--(axis cs:1.15915,8.16861237345016)
--(axis cs:1.20185,8.16861237345016)
--(axis cs:1.20185,8.2654172247258)
--(axis cs:1.29635,8.2654172247258)
--(axis cs:1.29635,8.37581473715754)
--(axis cs:1.4036,8.37581473715754)
--(axis cs:1.4036,8.52996468579557)
--(axis cs:1.5814,8.52996468579557)
--(axis cs:1.5814,8.704605865474)
--(axis cs:1.88535,8.704605865474)
--(axis cs:1.88535,8.88235631170357)
--(axis cs:2.37915,8.88235631170357)
--(axis cs:2.37915,9.0648324363241)
--(axis cs:3.1293,9.0648324363241)
--(axis cs:3.1293,9.13150991996058)
--(axis cs:3.1293,9.13150991996058)
--(axis cs:3.1293,9.13150991996058)
--(axis cs:13.1293,9.13150991996058)
--(axis cs:13.1293,9.13150991996058)
--(axis cs:13.1293,9.13150991996058)
--(axis cs:13.1293,0);

\path [draw=color1, fill=color1, opacity=0.1, very thin]
(axis cs:1.0791,0)
--(axis cs:1.0791,7.99429013865697)
--(axis cs:1.08885,7.99429013865697)
--(axis cs:1.08885,8.02755847224052)
--(axis cs:1.10855,8.02755847224052)
--(axis cs:1.10855,8.05428863622945)
--(axis cs:1.1329,8.05428863622945)
--(axis cs:1.1329,8.10699471053411)
--(axis cs:1.15915,8.10699471053411)
--(axis cs:1.15915,8.16861237345016)
--(axis cs:1.20185,8.16861237345016)
--(axis cs:1.20185,8.2654172247258)
--(axis cs:1.29635,8.2654172247258)
--(axis cs:1.29635,8.37581473715754)
--(axis cs:1.4036,8.37581473715754)
--(axis cs:1.4036,8.52996468579557)
--(axis cs:1.5814,8.52996468579557)
--(axis cs:1.5814,8.704605865474)
--(axis cs:1.88535,8.704605865474)
--(axis cs:1.88535,8.88235631170357)
--(axis cs:2.37915,8.88235631170357)
--(axis cs:2.37915,9.0648324363241)
--(axis cs:3.1293,9.0648324363241)
--(axis cs:3.1293,9.13150991996058)
--(axis cs:3.1293,9.13150991996058)
--(axis cs:3.1293,9.13150991996058)
--(axis cs:13.1293,9.13150991996058)
--(axis cs:13.1293,9.13150991996058)
--(axis cs:13.1293,0)
--(axis cs:13.1293,0)
--(axis cs:13.1293,0)
--(axis cs:3.1293,0)
--(axis cs:3.1293,0)
--(axis cs:3.1293,0)
--(axis cs:3.1293,0)
--(axis cs:2.37915,0)
--(axis cs:2.37915,0)
--(axis cs:1.88535,0)
--(axis cs:1.88535,0)
--(axis cs:1.5814,0)
--(axis cs:1.5814,0)
--(axis cs:1.4036,0)
--(axis cs:1.4036,0)
--(axis cs:1.29635,0)
--(axis cs:1.29635,0)
--(axis cs:1.20185,0)
--(axis cs:1.20185,0)
--(axis cs:1.15915,0)
--(axis cs:1.15915,0)
--(axis cs:1.1329,0)
--(axis cs:1.1329,0)
--(axis cs:1.10855,0)
--(axis cs:1.10855,0)
--(axis cs:1.08885,0)
--(axis cs:1.08885,0)
--(axis cs:1.0791,0)
--cycle;

\path [draw=color2, very thin]
(axis cs:1.0326,0)
--(axis cs:1.0326,7.90522221748678)
--(axis cs:1.064,7.90522221748678)
--(axis cs:1.064,8.09752068349911)
--(axis cs:1.10355,8.09752068349911)
--(axis cs:1.10355,8.3053802678758)
--(axis cs:1.15405,8.3053802678758)
--(axis cs:1.15405,8.49923639097998)
--(axis cs:1.2181,8.49923639097998)
--(axis cs:1.2181,8.69968084247663)
--(axis cs:1.46475,8.69968084247663)
--(axis cs:1.46475,8.91847279329954)
--(axis cs:1.6407,8.91847279329954)
--(axis cs:1.6407,9.0614045676246)
--(axis cs:1.83115,9.0614045676246)
--(axis cs:1.83115,9.21015880590953)
--(axis cs:2.06245,9.21015880590953)
--(axis cs:2.06245,9.3284458458292)
--(axis cs:2.37185,9.3284458458292)
--(axis cs:2.37185,9.37323458204225)
--(axis cs:2.37185,9.37323458204225)
--(axis cs:2.37185,9.37323458204225)
--(axis cs:12.37185,9.37323458204225)
--(axis cs:12.37185,9.37323458204225)
--(axis cs:12.37185,9.37323458204225)
--(axis cs:12.37185,0);

\path [draw=color2, fill=color2, opacity=0.1, very thin]
(axis cs:1.0326,0)
--(axis cs:1.0326,7.90522221748678)
--(axis cs:1.064,7.90522221748678)
--(axis cs:1.064,8.09752068349911)
--(axis cs:1.10355,8.09752068349911)
--(axis cs:1.10355,8.3053802678758)
--(axis cs:1.15405,8.3053802678758)
--(axis cs:1.15405,8.49923639097998)
--(axis cs:1.2181,8.49923639097998)
--(axis cs:1.2181,8.69968084247663)
--(axis cs:1.46475,8.69968084247663)
--(axis cs:1.46475,8.91847279329954)
--(axis cs:1.6407,8.91847279329954)
--(axis cs:1.6407,9.0614045676246)
--(axis cs:1.83115,9.0614045676246)
--(axis cs:1.83115,9.21015880590953)
--(axis cs:2.06245,9.21015880590953)
--(axis cs:2.06245,9.3284458458292)
--(axis cs:2.37185,9.3284458458292)
--(axis cs:2.37185,9.37323458204225)
--(axis cs:2.37185,9.37323458204225)
--(axis cs:2.37185,9.37323458204225)
--(axis cs:12.37185,9.37323458204225)
--(axis cs:12.37185,9.37323458204225)
--(axis cs:12.37185,0)
--(axis cs:12.37185,0)
--(axis cs:12.37185,0)
--(axis cs:2.37185,0)
--(axis cs:2.37185,0)
--(axis cs:2.37185,0)
--(axis cs:2.37185,0)
--(axis cs:2.06245,0)
--(axis cs:2.06245,0)
--(axis cs:1.83115,0)
--(axis cs:1.83115,0)
--(axis cs:1.6407,0)
--(axis cs:1.6407,0)
--(axis cs:1.46475,0)
--(axis cs:1.46475,0)
--(axis cs:1.2181,0)
--(axis cs:1.2181,0)
--(axis cs:1.15405,0)
--(axis cs:1.15405,0)
--(axis cs:1.10355,0)
--(axis cs:1.10355,0)
--(axis cs:1.064,0)
--(axis cs:1.064,0)
--(axis cs:1.0326,0)
--cycle;


\path [draw=color3, very thin]
(axis cs:1.0332,0)
--(axis cs:1.0332,7.96377695644185)
--(axis cs:1.06455,7.96377695644185)
--(axis cs:1.06455,8.16509279074437)
--(axis cs:1.11885,8.16509279074437)
--(axis cs:1.11885,8.33236331377999)
--(axis cs:1.17655,8.33236331377999)
--(axis cs:1.17655,8.5344152733388)
--(axis cs:1.2499,8.5344152733388)
--(axis cs:1.2499,8.72500297321082)
--(axis cs:1.5609,8.72500297321082)
--(axis cs:1.5609,8.91645480050354)
--(axis cs:1.7649,8.91645480050354)
--(axis cs:1.7649,9.06735652119834)
--(axis cs:1.99105,9.06735652119834)
--(axis cs:1.99105,9.18056096552133)
--(axis cs:2.26505,9.18056096552133)
--(axis cs:2.26505,9.26911336610963)
--(axis cs:2.6181,9.26911336610963)
--(axis cs:2.6181,9.28676600664873)
--(axis cs:2.6181,9.28676600664873)
--(axis cs:2.6181,9.28676600664873)
--(axis cs:12.6181,9.28676600664873)
--(axis cs:12.6181,9.28676600664873)
--(axis cs:12.6181,9.28676600664873)
--(axis cs:12.6181,0);
\path [draw=color3, fill=color3, opacity=0.1, very thin]
(axis cs:1.0332,0)
--(axis cs:1.0332,7.96377695644185)
--(axis cs:1.06455,7.96377695644185)
--(axis cs:1.06455,8.16509279074437)
--(axis cs:1.11885,8.16509279074437)
--(axis cs:1.11885,8.33236331377999)
--(axis cs:1.17655,8.33236331377999)
--(axis cs:1.17655,8.5344152733388)
--(axis cs:1.2499,8.5344152733388)
--(axis cs:1.2499,8.72500297321082)
--(axis cs:1.5609,8.72500297321082)
--(axis cs:1.5609,8.91645480050354)
--(axis cs:1.7649,8.91645480050354)
--(axis cs:1.7649,9.06735652119834)
--(axis cs:1.99105,9.06735652119834)
--(axis cs:1.99105,9.18056096552133)
--(axis cs:2.26505,9.18056096552133)
--(axis cs:2.26505,9.26911336610963)
--(axis cs:2.6181,9.26911336610963)
--(axis cs:2.6181,9.28676600664873)
--(axis cs:2.6181,9.28676600664873)
--(axis cs:2.6181,9.28676600664873)
--(axis cs:12.6181,9.28676600664873)
--(axis cs:12.6181,9.28676600664873)
--(axis cs:12.6181,0)
--(axis cs:12.6181,0)
--(axis cs:12.6181,0)
--(axis cs:2.6181,0)
--(axis cs:2.6181,0)
--(axis cs:2.6181,0)
--(axis cs:2.6181,0)
--(axis cs:2.26505,0)
--(axis cs:2.26505,0)
--(axis cs:1.99105,0)
--(axis cs:1.99105,0)
--(axis cs:1.7649,0)
--(axis cs:1.7649,0)
--(axis cs:1.5609,0)
--(axis cs:1.5609,0)
--(axis cs:1.2499,0)
--(axis cs:1.2499,0)
--(axis cs:1.17655,0)
--(axis cs:1.17655,0)
--(axis cs:1.11885,0)
--(axis cs:1.11885,0)
--(axis cs:1.06455,0)
--(axis cs:1.06455,0)
--(axis cs:1.0332,0)
--cycle;

\path [draw=color4, very thin]
(axis cs:1.28303333333333,0)
--(axis cs:1.28303333333333,8.24481358928613)
--(axis cs:1.28303333333333,8.26704724474991)
--(axis cs:1.38646666666667,8.26704724474991)
--(axis cs:1.38646666666667,8.38565088002783)
--(axis cs:1.5202,8.38565088002783)
--(axis cs:1.5202,8.51867568406122)
--(axis cs:1.73206666666667,8.51867568406122)
--(axis cs:1.73206666666667,8.69671561135512)
--(axis cs:2.08053333333333,8.69671561135512)
--(axis cs:2.08053333333333,8.87404096056643)
--(axis cs:2.59333333333333,8.87404096056643)
--(axis cs:2.59333333333333,9.0149146419155)
--(axis cs:3.3643,9.0149146419155)
--(axis cs:3.3643,9.07392878182218)
--(axis cs:3.3643,9.07392878182218)
--(axis cs:3.3643,9.07392878182218)
--(axis cs:13.3643,9.07392878182218)
--(axis cs:13.3643,9.07392878182218)
--(axis cs:13.3643,9.07392878182218)
--(axis cs:13.3643,0);
\path [draw=color4, fill=color4, opacity=0.1, very thin]
(axis cs:1.28303333333333,0)
--(axis cs:1.28303333333333,8.24481358928613)
--(axis cs:1.28303333333333,8.26704724474991)
--(axis cs:1.38646666666667,8.26704724474991)
--(axis cs:1.38646666666667,8.38565088002783)
--(axis cs:1.5202,8.38565088002783)
--(axis cs:1.5202,8.51867568406122)
--(axis cs:1.73206666666667,8.51867568406122)
--(axis cs:1.73206666666667,8.69671561135512)
--(axis cs:2.08053333333333,8.69671561135512)
--(axis cs:2.08053333333333,8.87404096056643)
--(axis cs:2.59333333333333,8.87404096056643)
--(axis cs:2.59333333333333,9.0149146419155)
--(axis cs:3.3643,9.0149146419155)
--(axis cs:3.3643,9.07392878182218)
--(axis cs:3.3643,9.07392878182218)
--(axis cs:3.3643,9.07392878182218)
--(axis cs:13.3643,9.07392878182218)
--(axis cs:13.3643,9.07392878182218)
--(axis cs:13.3643,0)
--(axis cs:13.3643,0)
--(axis cs:13.3643,0)
--(axis cs:3.3643,0)
--(axis cs:3.3643,0)
--(axis cs:3.3643,0)
--(axis cs:3.3643,0)
--(axis cs:2.59333333333333,0)
--(axis cs:2.59333333333333,0)
--(axis cs:2.08053333333333,0)
--(axis cs:2.08053333333333,0)
--(axis cs:1.73206666666667,0)
--(axis cs:1.73206666666667,0)
--(axis cs:1.5202,0)
--(axis cs:1.5202,0)
--(axis cs:1.38646666666667,0)
--(axis cs:1.38646666666667,0)
--(axis cs:1.28303333333333,0)
--(axis cs:1.28303333333333,0)
--(axis cs:7.74116666666667,0)
--cycle;

\addplot [semithick, color6, mark=diamond*, mark size=3, mark options={solid}, only marks]
table {%
1.70946666666667 9.24150081773772
1.7418 9.24716397124911
1.82996666666667 9.32438101525711
1.87186666666667 9.27024505428974
1.81463333333333 9.30669016219193
2.05873333333333 9.35679718539293
2.15626666666667 9.3872622751459
2.40886666666667 9.37770426487233
2.89306666666667 9.36420893583642
};

\addplot [semithick, color5, mark=diamond*, mark size=3, mark options={solid}, only marks]
table {%
1.27436666666667 8.85353733739286
1.32876666666667 8.93727766884469
1.24516666666667 8.80681256729337
1.41226666666667 9.04303071275202
1.3981 8.9941036427987
1.56496666666667 9.14534082773739
1.5919 9.1716418762417
1.8433 9.28647895403315
2.0214 9.30493881254364
};

==> tikzplotlib_figs_icmlcn/QPSK_Pareto_Lp2_data.tex <==
\path [draw=color1, very thin]
(axis cs:1.0791,0)
--(axis cs:1.0791,7.46771695350711)
--(axis cs:1.08885,7.46771695350711)
--(axis cs:1.08885,7.49535697285036)
--(axis cs:1.10855,7.49535697285036)
--(axis cs:1.10855,7.51479948582574)
--(axis cs:1.1329,7.51479948582574)
--(axis cs:1.1329,7.5571340290965)
--(axis cs:1.15915,7.5571340290965)
--(axis cs:1.15915,7.60492626877384)
--(axis cs:1.20185,7.60492626877384)
--(axis cs:1.20185,7.68026810453802)
--(axis cs:1.29635,7.68026810453802)
--(axis cs:1.29635,7.75999607403337)
--(axis cs:1.4036,7.75999607403337)
--(axis cs:1.4036,7.87318396255595)
--(axis cs:1.5814,7.87318396255595)
--(axis cs:1.5814,7.98875884382458)
--(axis cs:1.88535,7.98875884382458)
--(axis cs:1.88535,8.08705849319032)
--(axis cs:2.37915,8.08705849319032)
--(axis cs:2.37915,8.15324877048265)
--(axis cs:2.37915,8.15324877048265)
--(axis cs:2.37915,8.15324877048265)
--(axis cs:12.37915,8.15324877048265)
--(axis cs:12.37915,8.15324877048265)
--(axis cs:12.37915,8.15324877048265)
--(axis cs:12.37915,0);

\path [draw=color1, fill=color1, opacity=0.1, very thin]
(axis cs:1.0791,0)
--(axis cs:1.0791,7.46771695350711)
--(axis cs:1.08885,7.46771695350711)
--(axis cs:1.08885,7.49535697285036)
--(axis cs:1.10855,7.49535697285036)
--(axis cs:1.10855,7.51479948582574)
--(axis cs:1.1329,7.51479948582574)
--(axis cs:1.1329,7.5571340290965)
--(axis cs:1.15915,7.5571340290965)
--(axis cs:1.15915,7.60492626877384)
--(axis cs:1.20185,7.60492626877384)
--(axis cs:1.20185,7.68026810453802)
--(axis cs:1.29635,7.68026810453802)
--(axis cs:1.29635,7.75999607403337)
--(axis cs:1.4036,7.75999607403337)
--(axis cs:1.4036,7.87318396255595)
--(axis cs:1.5814,7.87318396255595)
--(axis cs:1.5814,7.98875884382458)
--(axis cs:1.88535,7.98875884382458)
--(axis cs:1.88535,8.08705849319032)
--(axis cs:2.37915,8.08705849319032)
--(axis cs:2.37915,8.15324877048265)
--(axis cs:2.37915,8.15324877048265)
--(axis cs:2.37915,8.15324877048265)
--(axis cs:12.37915,8.15324877048265)
--(axis cs:12.37915,8.15324877048265)
--(axis cs:12.37915,0)
--(axis cs:12.37915,0)
--(axis cs:12.37915,0)
--(axis cs:2.37915,0)
--(axis cs:2.37915,0)
--(axis cs:2.37915,0)
--(axis cs:2.37915,0)
--(axis cs:1.88535,0)
--(axis cs:1.88535,0)
--(axis cs:1.5814,0)
--(axis cs:1.5814,0)
--(axis cs:1.4036,0)
--(axis cs:1.4036,0)
--(axis cs:1.29635,0)
--(axis cs:1.29635,0)
--(axis cs:1.20185,0)
--(axis cs:1.20185,0)
--(axis cs:1.15915,0)
--(axis cs:1.15915,0)
--(axis cs:1.1329,0)
--(axis cs:1.1329,0)
--(axis cs:1.10855,0)
--(axis cs:1.10855,0)
--(axis cs:1.08885,0)
--(axis cs:1.08885,0)
--(axis cs:1.0791,0)
--cycle;


\path [draw=color2, very thin]
(axis cs:1.0326,0)
--(axis cs:1.0326,7.3987640226167)
--(axis cs:1.064,7.3987640226167)
--(axis cs:1.064,7.56142176301126)
--(axis cs:1.10355,7.56142176301126)
--(axis cs:1.10355,7.73575146703978)
--(axis cs:1.15405,7.73575146703978)
--(axis cs:1.15405,7.89382234147158)
--(axis cs:1.2181,7.89382234147158)
--(axis cs:1.2181,8.05471783857464)
--(axis cs:1.46475,8.05471783857464)
--(axis cs:1.46475,8.19878122074405)
--(axis cs:1.6407,8.19878122074405)
--(axis cs:1.6407,8.28417415465931)
--(axis cs:1.83115,8.28417415465931)
--(axis cs:1.83115,8.37035154248797)
--(axis cs:2.06245,8.37035154248797)
--(axis cs:2.06245,8.41910488182026)
--(axis cs:2.06245,8.41910488182026)
--(axis cs:2.06245,8.41910488182026)
--(axis cs:12.06245,8.41910488182026)
--(axis cs:12.06245,8.41910488182026)
--(axis cs:12.06245,8.41910488182026)
--(axis cs:12.06245,0);

\path [draw=color2, fill=color2, opacity=0.1, very thin]
(axis cs:1.0326,0)
--(axis cs:1.0326,7.3987640226167)
--(axis cs:1.064,7.3987640226167)
--(axis cs:1.064,7.56142176301126)
--(axis cs:1.10355,7.56142176301126)
--(axis cs:1.10355,7.73575146703978)
--(axis cs:1.15405,7.73575146703978)
--(axis cs:1.15405,7.89382234147158)
--(axis cs:1.2181,7.89382234147158)
--(axis cs:1.2181,8.05471783857464)
--(axis cs:1.46475,8.05471783857464)
--(axis cs:1.46475,8.19878122074405)
--(axis cs:1.6407,8.19878122074405)
--(axis cs:1.6407,8.28417415465931)
--(axis cs:1.83115,8.28417415465931)
--(axis cs:1.83115,8.37035154248797)
--(axis cs:2.06245,8.37035154248797)
--(axis cs:2.06245,8.41910488182026)
--(axis cs:2.06245,8.41910488182026)
--(axis cs:2.06245,8.41910488182026)
--(axis cs:12.06245,8.41910488182026)
--(axis cs:12.06245,8.41910488182026)
--(axis cs:12.06245,0)
--(axis cs:12.06245,0)
--(axis cs:12.06245,0)
--(axis cs:2.06245,0)
--(axis cs:2.06245,0)
--(axis cs:2.06245,0)
--(axis cs:2.06245,0)
--(axis cs:1.83115,0)
--(axis cs:1.83115,0)
--(axis cs:1.6407,0)
--(axis cs:1.6407,0)
--(axis cs:1.46475,0)
--(axis cs:1.46475,0)
--(axis cs:1.2181,0)
--(axis cs:1.2181,0)
--(axis cs:1.15405,0)
--(axis cs:1.15405,0)
--(axis cs:1.10355,0)
--(axis cs:1.10355,0)
--(axis cs:1.064,0)
--(axis cs:1.064,0)
--(axis cs:1.0326,0)
--cycle;

\path [draw=color3, very thin]
(axis cs:1.0332,0)
--(axis cs:1.0332,7.4505513962166)
--(axis cs:1.06455,7.4505513962166)
--(axis cs:1.06455,7.62122640183564)
--(axis cs:1.11885,7.62122640183564)
--(axis cs:1.11885,7.75623198779149)
--(axis cs:1.17655,7.75623198779149)
--(axis cs:1.17655,7.920842990417)
--(axis cs:1.2499,7.920842990417)
--(axis cs:1.2499,8.07122460039159)
--(axis cs:1.5609,8.07122460039159)
--(axis cs:1.5609,8.18292174903397)
--(axis cs:1.7649,8.18292174903397)
--(axis cs:1.7649,8.27361095089302)
--(axis cs:1.99105,8.27361095089302)
--(axis cs:1.99105,8.32166721561119)
--(axis cs:2.26505,8.32166721561119)
--(axis cs:2.26505,8.33942156812715)
--(axis cs:2.26505,8.33942156812715)
--(axis cs:2.26505,8.33942156812715)
--(axis cs:12.26505,8.33942156812715)
--(axis cs:12.26505,8.33942156812715)
--(axis cs:12.26505,8.33942156812715)
--(axis cs:12.26505,0);

\path [draw=color3, fill=color3, opacity=0.1, very thin]
(axis cs:1.0332,0)
--(axis cs:1.0332,7.4505513962166)
--(axis cs:1.06455,7.4505513962166)
--(axis cs:1.06455,7.62122640183564)
--(axis cs:1.11885,7.62122640183564)
--(axis cs:1.11885,7.75623198779149)
--(axis cs:1.17655,7.75623198779149)
--(axis cs:1.17655,7.920842990417)
--(axis cs:1.2499,7.920842990417)
--(axis cs:1.2499,8.07122460039159)
--(axis cs:1.5609,8.07122460039159)
--(axis cs:1.5609,8.18292174903397)
--(axis cs:1.7649,8.18292174903397)
--(axis cs:1.7649,8.27361095089302)
--(axis cs:1.99105,8.27361095089302)
--(axis cs:1.99105,8.32166721561119)
--(axis cs:2.26505,8.32166721561119)
--(axis cs:2.26505,8.33942156812715)
--(axis cs:2.26505,8.33942156812715)
--(axis cs:2.26505,8.33942156812715)
--(axis cs:12.26505,8.33942156812715)
--(axis cs:12.26505,8.33942156812715)
--(axis cs:12.26505,0)
--(axis cs:12.26505,0)
--(axis cs:12.26505,0)
--(axis cs:2.26505,0)
--(axis cs:2.26505,0)
--(axis cs:2.26505,0)
--(axis cs:2.26505,0)
--(axis cs:1.99105,0)
--(axis cs:1.99105,0)
--(axis cs:1.7649,0)
--(axis cs:1.7649,0)
--(axis cs:1.5609,0)
--(axis cs:1.5609,0)
--(axis cs:1.2499,0)
--(axis cs:1.2499,0)
--(axis cs:1.17655,0)
--(axis cs:1.17655,0)
--(axis cs:1.11885,0)
--(axis cs:1.11885,0)
--(axis cs:1.06455,0)
--(axis cs:1.06455,0)
--(axis cs:1.0332,0)
--cycle;

\path [draw=color4, very thin]
(axis cs:1.109166666666677,0)
--(axis cs:1.10916666666667,6.63452719199)
--(axis cs:1.10916666666667,7.48975325359715)
--(axis cs:1.1213,7.48975325359715)
--(axis cs:1.1213,7.51850725018948)
--(axis cs:1.15113333333333,7.51850725018948)
--(axis cs:1.15113333333333,7.53926143400062)
--(axis cs:1.17853333333333,7.53926143400062)
--(axis cs:1.17853333333333,7.57040046485803)
--(axis cs:1.21503333333333,7.57040046485803)
--(axis cs:1.21503333333333,7.62538182658307)
--(axis cs:1.28303333333333,7.62538182658307)
--(axis cs:1.28303333333333,7.67078294697599)
--(axis cs:1.38646666666667,7.67078294697599)
--(axis cs:1.38646666666667,7.75595734631373)
--(axis cs:1.5202,7.75595734631373)
--(axis cs:1.5202,7.84731851271134)
--(axis cs:1.73206666666667,7.84731851271134)
--(axis cs:1.73206666666667,7.96456274355658)
--(axis cs:2.08053333333333,7.96456274355658)
--(axis cs:2.08053333333333,8.05595947728055)
--(axis cs:2.59333333333333,8.05595947728055)
--(axis cs:2.59333333333333,8.08618578066173)
--(axis cs:2.59333333333333,8.08618578066173)
--(axis cs:2.59333333333333,8.08618578066173)
--(axis cs:12.5933333333333,8.08618578066173)
--(axis cs:12.5933333333333,8.08618578066173)
--(axis cs:12.5933333333333,8.08618578066173)
--(axis cs:12.5933333333333,0);
\path [draw=color4, fill=color4, opacity=0.1, very thin]
(axis cs:1.10916666666667,0)
--(axis cs:1.10916666666667,6.63452719199)
--(axis cs:1.10916666666667,7.48975325359715)
--(axis cs:1.1213,7.48975325359715)
--(axis cs:1.1213,7.51850725018948)
--(axis cs:1.15113333333333,7.51850725018948)
--(axis cs:1.15113333333333,7.53926143400062)
--(axis cs:1.17853333333333,7.53926143400062)
--(axis cs:1.17853333333333,7.57040046485803)
--(axis cs:1.21503333333333,7.57040046485803)
--(axis cs:1.21503333333333,7.62538182658307)
--(axis cs:1.28303333333333,7.62538182658307)
--(axis cs:1.28303333333333,7.67078294697599)
--(axis cs:1.38646666666667,7.67078294697599)
--(axis cs:1.38646666666667,7.75595734631373)
--(axis cs:1.5202,7.75595734631373)
--(axis cs:1.5202,7.84731851271134)
--(axis cs:1.73206666666667,7.84731851271134)
--(axis cs:1.73206666666667,7.96456274355658)
--(axis cs:2.08053333333333,7.96456274355658)
--(axis cs:2.08053333333333,8.05595947728055)
--(axis cs:2.59333333333333,8.05595947728055)
--(axis cs:2.59333333333333,8.08618578066173)
--(axis cs:2.59333333333333,8.08618578066173)
--(axis cs:2.59333333333333,8.08618578066173)
--(axis cs:12.5933333333333,8.08618578066173)
--(axis cs:12.5933333333333,8.08618578066173)
--(axis cs:12.5933333333333,0)
--(axis cs:12.5933333333333,0)
--(axis cs:12.5933333333333,0)
--(axis cs:2.59333333333333,0)
--(axis cs:2.59333333333333,0)
--(axis cs:2.59333333333333,0)
--(axis cs:2.59333333333333,0)
--(axis cs:2.08053333333333,0)
--(axis cs:2.08053333333333,0)
--(axis cs:1.73206666666667,0)
--(axis cs:1.73206666666667,0)
--(axis cs:1.5202,0)
--(axis cs:1.5202,0)
--(axis cs:1.38646666666667,0)
--(axis cs:1.38646666666667,0)
--(axis cs:1.28303333333333,0)
--(axis cs:1.28303333333333,0)
--(axis cs:1.21503333333333,0)
--(axis cs:1.21503333333333,0)
--(axis cs:1.17853333333333,0)
--(axis cs:1.17853333333333,0)
--(axis cs:1.15113333333333,0)
--(axis cs:1.15113333333333,0)
--(axis cs:1.1213,0)
--(axis cs:1.1213,0)
--(axis cs:1.10916666666667,0)
--(axis cs:1.10916666666667,0)
--(axis cs:7.74116666666667,0)
--cycle;


\addplot [semithick, color6, mark=diamond*, mark size=3, mark options={solid}, only marks]
table {%
1.30253333333333 8.21295835047727
1.36876666666667 8.23252111187093
1.33133333333333 8.25580044063302
1.41016666666667 8.30284305607452
1.41243333333333 8.31721198686378
1.46193333333333 8.33214694974514
1.62623333333333 8.4089492541961
1.67953333333333 8.39972896473932
2.23913333333333 8.40502126524374
};

\addplot [semithick, color5, mark=diamond*, mark size=3, mark options={solid}, only marks]
table {%
1.12583333333333 7.86343004646802
1.15706666666667 7.97500983356438
1.118 7.88747017668727
1.19526666666667 8.05164702432909
1.15303333333333 7.95375619089119
1.2631 8.13814228099469
1.333 8.2603913347467
1.47343333333333 8.31941640893119
1.65126666666667 8.39330235887486
};
